UPIR: Toward the Design of Unified Parallel Intermediate Representation for Parallel Programming Models

The complexity of heterogeneous computing architectures, as well as the demand for productive and portable parallel application development, have driven the evolution of parallel programming models to become more comprehensive and complex than before. Enhancing the conventional compilation technologies and software infrastructure to be parallelism-aware has become one of the main goals of recent compiler development. In this paper, we propose the design of unified parallel intermediate representation (UPIR) for multiple parallel programming models and for enabling unified compiler transformation for the models. UPIR specifies three commonly used parallelism patterns (SPMD, data and task parallelism), data attributes and explicit data movement and memory management, and synchronization operations used in parallel programming. We demonstrate UPIR via a prototype implementation in the ROSE compiler for unifying IR for both OpenMP and OpenACC and in both C/C++ and Fortran, for unifying the transformation that lowers both OpenMP and OpenACC code to LLVM runtime, and for exporting UPIR to LLVM MLIR dialect.

==> src/related.tex <==
\subsection{task graph for visualization}
Task graph is a direct acyclic graph (DAG) model~\cite{kwok1999benchmarking} which can be derived from early age researches.
On the one hand, task graph is used as DAG scheduling algorithms(DSAs).
It is applied to serial programs or desired tasks to generate an optimized computation structure, such as parallelism and task dependency.
As the work presented by Coffman and Graham~\cite{coffman1972optimal}, the so-called task graph is used for scheduling given computations on two-processor systems.
Then this idea is also extended to scheduling in general-purpose distributed computation systems~\cite{casavant1988taxonomy}.

On the other hand, tools/frameworks are developed based on task graph to analysis parallelism or task dependency.
This idea is applied to both serial programs and distributed computation system based programs such as programs implemented with multi-threads and/or multi-processors.
It goes to the opposite way comparing with DSAs, and it covers almost all the aspects including visualization that the parallelism and task dependency can be optimized.
There are language specific ones, for instance, Grain Graph~\cite{muddukrishna2016grain} presents a OpenMP specific performance analysis method.
This method concentrates on tasks and parallel for-loops.
Pollock et.al~\cite{pollockprogram} shows MPI specific program flow graph construction.

For visualization, task graph presents decent illustration to users to review visualized program in distributed computation system and to see the potential of optimization.
HPCTOOLKIT~\cite{adhianto2010hpctoolkit} is an integrated suite of tools visualizing optimized serial or parallel programs based on call path profiling and tracing.
DAGViz~\cite{huynh2015dagviz} visualizes execution of task parallel program with DAGs to analysis performance.
Within the DAGs, hierarchical structure and huge numbers of nodes are handled properly.

Our work is enhanced from visualization usage of task graph, and we are trying to present informative parallel flow graphs to users.
We think about the interactive graph as well given that the dot graph file can be connected to html index with HTML language or JavaScript.

\subsection{MLIR}

\todo {Describe MLIR and its application}
